Model Selection with a Shapelet-based Distance Measure for Multi-source Transfer Learning in Time Series Classification

Transfer learning is a common practice that alleviates the need for extensive data to train neural networks. It is performed by pre-training a model using a source dataset and fine-tuning it for a target task. However, not every source dataset is appropriate for each target dataset, especially for time series. In this paper, we propose a novel method of selecting and using multiple datasets for transfer learning for time series classification. Specifically, our method combines multiple datasets as one source dataset for pre-training neural networks. Furthermore, for selecting multiple sources, our method measures the transferability of datasets based on shapelet discovery for effective source selection. While traditional transferability measures require considerable time for pre-training all the possible sources for source selection of each possible architecture, our method can be repeatedly used for every possible architecture with a single simple computation. Using the proposed method, we demonstrate that it is possible to increase the performance of temporal convolutional neural networks (CNN) on time series datasets.

==> mybibwithdoi.tex <==


@inproceedings{iwana2016robust,
  title={A Robust Dissimilarity-based Neural Network for Temporal Pattern Recognition},
  author={Iwana, Brian Kenji and Frinken, Volkmar and Uchida, Seiichi},
  booktitle={Int. Conf. Frontiers in Handwriting Recogn.},
  year={2016},
  pages={265--270},
  doi={10.1109/ICFHR.2016.0058},
}

@article{karim2017lstm,
  title={LSTM fully convolutional networks for time series classification},
  author={Karim, Fazle and Majumdar, Somshubra and Darabi, Houshang and Chen, Shun},
  journal={IEEE Access},
  volume={6},
  pages={1662--1669},
  year={2017},
  publisher={IEEE}
}

@article{ismail2019deep,
  title={Deep learning for time series classification: a review},
  author={Ismail Fawaz, Hassan and Forestier, Germain and Weber, Jonathan and Idoumghar, Lhassane and Muller, Pierre-Alain},
  journal={Data mining and knowledge discovery},
  volume={33},
  number={4},
  pages={917--963},
  year={2019},
  publisher={Springer}
}

@article{Middlehurst_2021, title={HIVE-COTE 2.0: a new meta ensemble for time series classification}, volume={110}, 
DOI={10.1007/s10994-021-06057-9}, number={11–12}, journal={Machine Learning}, publisher={Springer}, author={Middlehurst, Matthew and Large, James and Flynn, Michael and Lines, Jason and Bostrom, Aaron and Bagnall, Anthony}, year={2021}, pages={3211–3243} }

@inproceedings{Ismail_Fawaz_2018,
	doi = {10.1109/bigdata.2018.8621990},
	year = 2018,
	author = {Hassan Ismail Fawaz and Germain Forestier and Jonathan Weber and Lhassane Idoumghar and Pierre-Alain Muller},
	title = {Transfer learning for time series classification},
	booktitle = {{IEEE} ICBD}
}

@article{bai2018empirical,
  title={An empirical evaluation of generic convolutional and recurrent networks for sequence modeling},
  author={Bai, Shaojie and Kolter, J Zico and Koltun, Vladlen},
  journal={arXiv preprint arXiv:1803.01271},
  year={2018}
}

@article{iwana2021an,
  title={An Empirical Survey of Data Augmentation for Time Series Classification with Neural Networks},
  author={Iwana, Brian Kenji and Uchida, Seiichi},
  journal={PLOS ONE},
  year={2021},
  doi={10.1371/journal.pone.0254841},
}

@article{zhuang2020comprehensive,
  title={A comprehensive survey on transfer learning},
  author={Zhuang, Fuzhen and Qi, Zhiyuan and Duan, Keyu and Xi, Dongbo and Zhu, Yongchun and Zhu, Hengshu and Xiong, Hui and He, Qing},
  journal={Proc. IEEE},
  volume={109},
  number={1},
  pages={43--76},
  year={2020},
  publisher={IEEE}
}

@article{Lecun_1998,
	doi = {10.1109/5.726791},
	year = 1998,
	publisher = {IEEE},
	volume = {86},
	number = {11},
	pages = {2278--2324},
	author = {Y. Lecun and L. Bottou and Y. Bengio and P. Haffner},
	title = {Gradient-based learning applied to document recognition},
	journal = {Proc. {IEEE}}
}


@inproceedings{Wang_2017,
	doi = {10.1109/ijcnn.2017.7966039},
	year = 2017,
	author = {Zhiguang Wang and Weizhong Yan and Tim Oates},
	title = {Time series classification from scratch with deep neural networks: A strong baseline},
	booktitle = {IJCNN}
}

@article{cui2016multi,
  title={Multi-scale convolutional neural networks for time series classification},
  author={Cui, Zhicheng and Chen, Wenlin and Chen, Yixin},
  journal={arXiv preprint arXiv:1603.06995},
  year={2016}
}

@inproceedings{serra2018towards,
  title={Towards a universal neural network encoder for time series},
  author={Serra, Joan and Pascual, Santiago and Karatzoglou, Alexandros},
  booktitle={Artificial Intelligence Research and Development},
  pages={120--129},
  year={2018},
  publisher={IOS Press}
}

@inproceedings{Dridi_2021,
	doi = {10.1109/icc42927.2021.9500507},
	year = 2021,
	author = {Aicha Dridi and Hossam Afifi and Hassine Moungla and Cherifa Boucetta},
	title = {Transfer Learning for Classification and Prediction of Time Series for Next Generation Networks},
	booktitle = {{IEEE} ICC}
}

@article{Li_2020,
	doi = {10.3390/s20154271},
	year = 2020,
	publisher = {{MDPI}},
	volume = {20},
	number = {15},
	pages = {4271},
	author = {Fr{\'{e}}d{\'{e}}ric Li and Kimiaki Shirahama and Muhammad Adeel Nisar and Xinyu Huang and Marcin Grzegorzek},
	title = {Deep Transfer Learning for Time Series Data Based on Sensor Modality Classification},
	journal = {Sensors}
}

@inproceedings{Clark_2022,
	doi = {10.1109/ccece49351.2022.9918279},
	year = 2022,
	author = {Ryan Clark and Thomas E. Doyle},
	title = {A Priori Quantification of Transfer Learning Performance on Time Series Classification for Cyber-Physical Health Systems},
	booktitle = {{IEEE} CCECE}
}

@inproceedings{Gikunda_2021,
	doi = {10.1109/icmla52953.2021.00129},
	year = 2021,
	author = {Patrick Gikunda and Nicolas Jouandeau},
	title = {Homogeneous Transfer Active Learning for Time Series Classification},
	booktitle = {{IEEE} ICMLA}
}

@article{Petitjean_2011,
	doi = {10.1016/j.patcog.2010.09.013},
	year = 2011,
	publisher = {Elsevier},
	volume = {44},
	number = {3},
	pages = {678--693},
	author = {Fran{\c{c}}ois Petitjean and Alain Ketterlin and Pierre Gan{\c{c}}arski},
	title = {A global averaging method for dynamic time warping, with applications to clustering},
	journal = {Pattern Recognition}
}

 @misc{UCRArchive2018,
        title = {The UCR Time Series Classification Archive},
        author = {Dau, Hoang Anh and Keogh, Eamonn and Kamgar, Kaveh and Yeh, Chin-Chia Michael and Zhu, Yan and Gharghabi, Shaghayegh and Ratanamahatana, Chotirat Ann and Yanping and Hu, Bing 
                  and Begum, Nurjahan and Bagnall, Anthony and Mueen, Abdullah and Batista, Gustavo and Hexagon-ML},
        year = {2018},
        month = {October},
        note = {https://www.cs.ucr.edu/~eamonn/time\_series\_data\_2018/}
    }


@inproceedings{Yeh_2016,
	doi = {10.1109/icdm.2016.0179},
	year = 2016,
	author = {Chin-Chia Michael Yeh and Yan Zhu and Liudmila Ulanova and Nurjahan Begum and Yifei Ding and Hoang Anh Dau and Diego Furtado Silva and Abdullah Mueen and Eamonn Keogh},
	title = {Matrix Profile I: All Pairs Similarity Joins for Time Series: A Unifying View That Includes Motifs, Discords and Shapelets},
	booktitle = {IEEE ICDM}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={CVPR},
  pages={248--255},
  year={2009},
}



@inproceedings{Ye_2009,
	doi = {10.1145/1557019.1557122},
	year = 2009,
	author = {Lexiang Ye and Eamonn Keogh},
	title = {Time series shapelets},
	booktitle = {ACM KDD}
}

@InProceedings{pmlr-v119-nguyen20b,
  title = 	 {{LEEP}: A New Measure to Evaluate Transferability of Learned Representations},
  author =       {Nguyen, Cuong and Hassner, Tal and Seeger, Matthias and Archambeau, Cedric},
  booktitle = 	 {ICML},
  pages = 	 {7294--7305},
  year = 	 {2020},
}

@inproceedings{Tran_2019,
	doi = {10.1109/iccv.2019.00148},
	year = 2019,
	author = {Anh Tran and Cuong Nguyen and Tal Hassner},
	title = {Transferability and Hardness of Supervised Classification Tasks},
	booktitle = {ICCV}
}


@InProceedings{pmlr-v162-huang22d,
  title = 	 {Frustratingly Easy Transferability Estimation},
  author =       {Huang, Long-Kai and Huang, Junzhou and Rong, Yu and Yang, Qiang and Wei, Ying},
  booktitle = 	 {ICML},
  pages = 	 {9201--9225},
  year = 	 {2022},
}


@InProceedings{pmlr-v139-you21b,
  title = 	 {LogME: Practical Assessment of Pre-trained Models for Transfer Learning},
  author =       {You, Kaichao and Liu, Yong and Wang, Jianmin and Long, Mingsheng},
  booktitle = 	 {ICML},
  pages = 	 {12133--12143},
  year = 	 {2021},
}

@inproceedings{tanisaro2016time,
  title={Time series classification using time warping invariant echo state networks},
  author={Tanisaro, Pattreeya and Heidemann, Gunther},
  booktitle={IEEE ICMLA},
  pages={831--836},
  year={2016},
}

@inproceedings{le2016data,
  title={Data augmentation for time series classification using convolutional neural networks},
  author={Le Guennec, Arthur and Malinowski, Simon and Tavenard, Romain},
  booktitle={ECML/PKDD WAALTD},
  year={2016}
}

@inproceedings{Bao_2019,
	doi = {10.1109/icip.2019.8803726},
	year = 2019,
	author = {Yajie Bao and Yang Li and Shao-Lun Huang and Lin Zhang and Lizhong Zheng and Amir Zamir and Leonidas Guibas},
	title = {An Information-Theoretic Approach to Transferability in Task Transfer Learning},
	booktitle = {ICIP}
}

@article{Zhuang_2021,
	doi = {10.1109/jproc.2020.3004555},
	year = 2021,
	publisher = {IEEE},
	volume = {109},
	number = {1},
	pages = {43--76},
	author = {Fuzhen Zhuang and Zhiyuan Qi and Keyu Duan and Dongbo Xi and Yongchun Zhu and Hengshu Zhu and Hui Xiong and Qing He},
	title = {A Comprehensive Survey on Transfer Learning},
	journal = {Proceed. {IEEE}}
}

@inproceedings{Yao_2010,
	doi = {10.1109/cvpr.2010.5539857},
	year = 2010,
	author = {Yi Yao and Gianfranco Doretto},
	title = {Boosting for transfer learning with multiple sources},
	booktitle = {IEEE CVPR}
}

@article{Huang_2012,
	doi = {10.1016/j.patrec.2011.11.023},
	year = 2012,
	publisher = {Elsevier},
	volume = {33},
	number = {5},
	pages = {568--579},
	author = {Pipei Huang and Gang Wang and Shiyin Qin},
	title = {Boosting for transfer learning from multiple data sources},
	journal = {Pattern Recognition Letters}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, D. P. and Ba, J.},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@article{Schuster_1997,
	doi = {10.1109/78.650093},
	year = 1997,
	publisher = {IEEE},
	volume = {45},
	number = {11},
	pages = {2673--2681},
	author = {M. Schuster and K.K. Paliwal},
	title = {Bidirectional recurrent neural networks},
	journal = {{IEEE} Transactions on Signal Processing}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT press}
}

@article{fawaz2018data,
  title={Data augmentation using synthetic data for time series classification with deep residual networks},
  author={Fawaz, Hassan Ismail and Forestier, Germain and Weber, Jonathan and Idoumghar, Lhassane and Muller, Pierre-Alain},
  journal={arXiv preprint arXiv:1808.02455},
  year={2018}
}

@inproceedings{Tan_2013,
	doi = {10.1137/1.9781611972832.27},
	year = 2013,
	author = {Ben Tan and Erheng Zhong and Evan Wei Xiang and Qiang Yang},
	title = {Multi-Transfer: Transfer Learning with Multiple Views and Multiple Sources},
	booktitle = {SIAM ICDM}
}

@article{Song_2017,
	doi = {10.1007/s00500-017-2755-8},
	year = 2017,
	publisher = {Springer },
	volume = {22},
	number = {24},
	pages = {8107--8118},
	author = {Hyun-Je Song and Seong-Bae Park},
	title = {Identifying intention posts in discussion forums using multi-instance learning and multiple sources transfer learning},
	journal = {Soft Computing}
}

@article{Weber_2021,
	doi = {10.1109/access.2021.3134628},
	year = 2021,
	publisher = {IEEE},
	volume = {9},
	pages = {165409--165432},
	author = {Manuel Weber and Maximilian Auch and Christoph Doblander and Peter Mandl and Hans-Arno Jacobsen},
	title = {Transfer Learning With Time Series Data: A Systematic Mapping Study},
	journal = {{IEEE} Access}
}

@article{Thompson_2022,
	doi = {10.2139/ssrn.4214809},
	year = 2022,
	publisher = {Elsevier},
	author = {Aaron Thompson},
	title = {Transfer Learning with Time Series Prediction: Review},
	journal = {{SSRN} Electronic Journal}
}

@article{Li_2019,
	doi = {10.1109/tcyb.2019.2904052},
	year = 2019,
	publisher = {IEEE},
	pages = {1--13},
	author = {Jinpeng Li and Shuang Qiu and Yuan-Yuan Shen and Cheng-Lin Liu and Huiguang He},
	title = {Multisource Transfer Learning for Cross-Subject {EEG} Emotion Recognition},
	journal = {{IEEE} Transactions on Cybernetics}
}

@article{SAKOE_1990,
	doi = {10.1016/b978-0-08-051584-7.50016-4},
	year = 1990,
	publisher = {Elsevier},
	pages = {159--165},
	author = {HIROAKI SAKOE and SEIBI CHIBA},
	title = {Dynamic Programming Algorithm Optimization for Spoken Word Recognition},
	journal = {Readings in Speech Recognition}
}

@inproceedings{Ren_2022,
	doi = {10.1109/icicml57342.2022.10009876},
	year = 2022,
	author = {Run Ren and Yameng Yang and Hailong Ren},
	title = {{EEG} Emotion Recognition using Multisource Instance Transfer Learning Framework},
	booktitle = {ICICML}
}

@article{Ye_2021,
	doi = {10.1016/j.patcog.2020.107617},
	year = 2021,
	publisher = {Elsevier},
	volume = {109},
	pages = {107617},
	author = {Rui Ye and Qun Dai},
	title = {Implementing transfer learning across different datasets for time series forecasting},
	journal = {Pattern Recognition}
}

@article{menendez1997jensen,
  title={The jensen-shannon divergence},
  author={Men{\'e}ndez, ML and Pardo, JA and Pardo, L and Pardo, MC},
  journal={Journal of the Franklin Institute},
  volume={334},
  number={2},
  pages={307--318},
  year={1997},
  publisher={Elsevier}
}

@inproceedings{Wang_2018,
	doi = {10.1145/3265689.3265705},
	year = 2018,
	author = {Jindong Wang and Vincent W. Zheng and Yiqiang Chen and Meiyu Huang},
	title = {Deep Transfer Learning for Cross-domain Activity Recognition},
	booktitle = {ICCSE}
}

@inproceedings{Dai_2007,
	doi = {10.1145/1273496.1273521},
	year = 2007,
	author = {Wenyuan Dai and Qiang Yang and Gui-Rong Xue and Yong Yu},
	title = {Boosting for transfer learning},
	booktitle = {ICML}
}

@inproceedings{Lotte_2010,
	doi = {10.1109/icassp.2010.5495183},
	year = 2010,
	author = {Fabien Lotte and Cuntai Guan},
	title = {Learning from other subjects helps reducing Brain-Computer Interface calibration time},
	booktitle = {IEEE ICASSP}
}

@misc{simonyan2015deep,
      title={Very Deep Convolutional Networks for Large-Scale Image Recognition}, 
      author={Karen Simonyan and Andrew Zisserman},
      year={2015},
      eprint={1409.1556},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

 @article{Rebbapragada_2008, title={Finding anomalous periodic time series: An application to catalogs of periodic variable stars}, volume={74}, ISSN={1573-0565}, DOI={10.1007/s10994-008-5093-3}, number={3}, journal={Machine Learning}, publisher={Springer}, author={Rebbapragada, Umaa and Protopapas, Pavlos and Brodley, Carla E. and Alcock, Charles}, year={2008}, month=dec, pages={281–313}}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{ye2021implementing,
  title={Implementing transfer learning across different datasets for time series forecasting},
  author={Ye, Rui and Dai, Qun},
  journal={Pattern Recognition},
  volume={109},
  pages={107617},
  year={2021},
  publisher={Elsevier}
}

@article{lu2023multi,
  title={A multi-source transfer learning model based on LSTM and domain adaptation for building energy prediction},
  author={Lu, Huiming and Wu, Jiazheng and Ruan, Yingjun and Qian, Fanyue and Meng, Hua and Gao, Yuan and Xu, Tingting},
  journal={International Journal of Electrical Power \& Energy Systems},
  volume={149},
  pages={109024},
  year={2023},
  publisher={Elsevier}
}
